SG-UMP: Sequence-Guided Universal Multimodal Prioritization Calculation Framework

Multimodal sequential recommendation (MSR) improves recommendation by incorporating heterogeneous information such as text, images, and user interactions. However, existing MSR methods often fail to capture user-level preference heterogeneity and dataset-level modality bias, limiting their adaptability across users and datasets. To address this issue, we propose \textbf{S}equence-\textbf{G}uided \textbf{U}niversal \textbf{M}ultimodal \textbf{P}rioritization Calculation Framework (\textbf{SG-UMP}), a plug-and-play plugin for enhancing multimodal information processing in MSR. SG-UMP includes a Module Combiner for flexible multimodal processing and a Module Router for dynamic module ordering, enabling adaptation to both user preferences and dataset characteristics. Experiments on four real-world datasets show that SG-UMP consistently improves recommendation performance across different backbones and multimodal settings. The code is available at https://github.com/esemsc-xz524/SG-UMP .

==> X-table.tex <==
\begin{table*}[!ht]
\caption{Validation of Module Importance and Sequence Effect on Model Performance. The best performance is highlighted in bold. The table has two parts: (1) The importance and impact of different modules. \underline{$w/o$ Filter}: Excluding the Frequency Filter Layer. \underline{$w/o$ Attention}: Excluding Hierarchical Attention Layer. \underline{$w/o$ MOE}: Excluding the Multi-Scale Fusion Layer. (2) The effect of different module sequence combinations. (a) is Frequency Filter Layer, (b) is Hierarchical Attention Layer, and (c) is Multi-Scale Fusion Layer. All results are averaged over 5 runs per dataset to ensure statistical robustness and are statistically significant with \(p < 0.05\).}

\centering
\resizebox{0.96\textwidth}{!}{%
\begin{tabular}{cc ccccc | cc cccccc}
\toprule
\multicolumn{7}{c|}{(1) The Importance and Effect of different Module.} & \multicolumn{8}{c}{(2) The Importance and Effect of different Module Sequence.} \\\hline
Datasets& Metric & STOSA & $w/o$ Filter & $w/o$ Attention & $w/o$ MOE & SG-UMP+STOSA & Datasets& Metrics & a-b-c  & a-c-b & b-a-c & b-c-a & c-a-b & c-b-a \\\hline
\multirow{4}{*}{Home} 
& R@10  & 0.0169 & 0.0216 & 0.0213 & 0.0227 & \textbf{0.0242}& \multirow{4}{*}{Home}   & R@10 & 0.0239 & 0.0227 & 0.0229 & 0.0214 & 0.0229 & \textbf{0.0242}\\
& R@20  & 0.0264 & 0.0316 & 0.0314 & 0.0322 & \textbf{0.0349}&                         & R@20 & 0.0333 & 0.0328 & 0.0329 & 0.0319 & 0.0333 & \textbf{0.0349}\\
& N@10  & 0.0098 & 0.0121 & 0.0120 & 0.0124 & \textbf{0.0144}&                         & N@10 & 0.0121 & 0.0138 & 0.0133 & 0.0140 & 0.0131 & \textbf{0.0144}\\
& N@20  & 0.0113 & 0.0134 & 0.0132 & 0.0141 & \textbf{0.0167}&                         & N@20 & 0.0162 & 0.0144 & 0.0158 & 0.0146 & 0.0156 & \textbf{0.0167}\\\hline

\multirow{4}{*}{Beauty} 
& R@10  & 0.0648 & 0.0726 & 0.0723 & 0.0725 & \textbf{0.0788}& \multirow{4}{*}{Beauty} & R@10 & 0.0779 & 0.0774 & \textbf{0.0788} & 0.0780 & 0.0785 & 0.0766\\ 
& R@20  & 0.0941 & 0.1028 & 0.1021 & 0.1024 & \textbf{0.1091}&                         & R@20 & 0.1066 & 0.1073 & \textbf{0.1091} & 0.1083 & 0.1067 & 0.1026\\ 
& N@10  & 0.0339 & 0.0406 & 0.0408 & 0.0403 & \textbf{0.0455}&                         & N@10 & 0.0436 & 0.0449 & \textbf{0.0455} & 0.0443 & 0.0436 & 0.0446\\ 
& N@20  & 0.0385 & 0.0431 & 0.0433 & 0.0434 & \textbf{0.0534}&                         & N@20 & 0.0525 & 0.0524 & \textbf{0.0534} & 0.0512 & 0.0517 & 0.0532\\\hline 

\multirow{4}{*}{Office} 
& R@10  & 0.0904 & 0.0926 & 0.0923 & 0.0915 & \textbf{0.0975}& \multirow{4}{*}{Office} & R@10 & 0.0889 & \textbf{0.0975} & 0.0913 & 0.0922 & 0.0869 & 0.0922\\
& R@20  & 0.1388 & 0.1376 & 0.1382 & 0.1374 & \textbf{0.1454}&                         & R@20 & 0.1372 & \textbf{0.1454} & 0.1319 & 0.1425 & 0.1295 & 0.1394\\
& N@10  & 0.0516 & 0.0521 & 0.0520 & 0.0523 & \textbf{0.0563}&                         & N@10 & 0.0502 & \textbf{0.0563} & 0.0516 & 0.0535 & 0.0499 & 0.0527\\
& N@20  & 0.0626 & 0.0621 & 0.0623 & 0.0618 & \textbf{0.0683}&                         & N@20 & 0.0622 & \textbf{0.0683} & 0.0619 & 0.0661 & 0.0606 & 0.0645\\\hline

\multirow{4}{*}{Yelp} 
& R@10  & 0.0248 & 0.0256 & 0.0253 & 0.0255 & \textbf{0.0279}& \multirow{4}{*}{Yelp}   & R@10 & \textbf{0.0266} & 0.0256 & 0.0244 & 0.0233 & 0.0263 & 0.0245\\
& R@20  & 0.0424 & 0.0446 & 0.0444 & 0.0441 & \textbf{0.0492}&                         & R@20 & \textbf{0.0442} & 0.0433 & 0.0407 & 0.0391 & 0.0439 & 0.0405\\
& N@10  & 0.0128 & 0.0134 & 0.0136 & 0.0131 & \textbf{0.0151}&                         & N@10 & \textbf{0.0132} & 0.0128 & 0.0121 & 0.0114 & 0.0129 & 0.0120\\
& N@20  & 0.0161 & 0.0167 & 0.0165 & 0.0165 & \textbf{0.0184}&                         & N@20 & \textbf{0.0177} & 0.0172 & 0.0162 & 0.0154 & 0.0173 & 0.0160\\\hline
\end{tabular}
}
\label{tab:preciple1&2}
\end{table*}

==> Y-table.tex <==
\begin{table*}[!ht]
    \small
    \setlength\tabcolsep{2pt}
    \caption{Performance comparison with three groups of baselines. The best performance is highlighted in bold, and the second best is highlighted by underlines. \emph{vs. Vanilla} represents the relative improvements over the vanilla. \emph{vs. Best} represents the relative improvements over the best baseline in percentage. All results are averaged over 5 runs per dataset to ensure statistical robustness and are statistically significant with \(p < 0.05\).}
    \label{tab:compare}
    \vspace{-5pt}
    \resizebox{0.96\linewidth}{!}{
        \begin{tabular}{c|cccc|cccc|cccc|cccc}
        \hline
        \makebox[0.15\linewidth]{Datasets}        & \multicolumn{4}{c|}{Home}                                                         & \multicolumn{4}{c|}{Beauty}                                                                                           & \multicolumn{4}{c|}{Office}                                                                                          & \multicolumn{4}{c}{Yelp}                                                                             \\ \hline
        Metric                                    & {R@10}          & {R@20}           & {N@10}          &{N@20}                      & {R@10}                      & {R@20}                      & {N@10}                      & {N@20}                      & {R@10}                       & {R@20}                     & {N@10}                    & {N@20}                       & {R@10}                            & {R@20}                          & {N@10}               & {N@20}  \\ \hline
        SASRec (ICDM'18)                          & 0.0168          & 0.0249           & 0.0081          & 0.0099                     & 0.0534                      & 0.0839                      & 0.0247                      & 0.0332                      & 0.0853& 0.1256& 0.0487& 0.0592& 0.0233                            & 0.0391                          & 0.0123               & 0.0152  \\
        BERT4Rec (CIKM'19)                        & 0.0156          & 0.0238           & 0.0073          & 0.0101                     & 0.0545                      & 0.0852                      & 0.0254                      & 0.0351                      & 0.0857& 0.1232& 0.0462& 0.0599& 0.0245                            & 0.0411                          & 0.0119               & 0.0162  \\ 
        LightGCN (SIGIR'20)                       & 0.0161          & 0.0243           & 0.0077          & 0.0103                     & 0.0549                      & 0.0861                      & 0.0258                      & 0.0355                      & 0.0866& 0.1215& 0.0463& 0.0602& 0.0236                            & 0.0414                          & 0.0123               & 0.0166  \\
        STOSA (WWW'22)                            & 0.0169          & 0.0264           & 0.0098          & 0.0113                     & 0.0648                      & 0.0941                      & 0.0339                      & 0.0385                      & 0.0864& 0.1284& 0.0497& 0.0602& 0.0238                            & 0.0424                          & 0.0128               & 0.0161  \\
        FMLPRec (WWW'22)                          & 0.0178          & 0.0268           & 0.0085          & 0.0108                     & 0.0654                      & 0.0961                      & 0.0348                      & 0.0381                      & 0.0881& 0.1321& 0.0488& 0.0601& 0.0247                            & 0.0438                          & 0.0131               & 0.0167  \\
        Oracle4Rec (WSDM'25)                          & 0.0211          & 0.0302           & 0.0131          & 0.0144                     & 0.0686                      & 0.0997                      & 0.0379                      & 0.0451                      & {\ul 0.0901}& {\ul 0.1419}& {\ul 0.0511}& 0.0610& 0.0266                            & 0.0445                          & 0.0146               & 0.0175  \\ \hline
        VBPR (AAAI'16)                            & 0.0159          & 0.0256           & 0.0074          & 0.0095                     & 0.0551                      & 0.0842                      & 0.0252                      & 0.0337                      & 0.0821& 0.1212& 0.0459& 0.0565& 0.0237                            & 0.0434                          & 0.0123               & 0.0163  \\
        MMMLP (WWW'23)                            & 0.0209          & 0.0293           & 0.0124          & 0.0134                     & 0.0671                      & 0.0979                      & 0.0387                      & 0.0441                      & 0.0872& 0.1291& 0.0501& 0.0603& 0.0254                            & 0.0452                          & 0.0138               & 0.0169  \\
        MML (CIKM'23)                             & {\ul 0.0237}    & 0.0327           & {\ul 0.0145}          & 0.0149                     & {\ul 0.0735}                & 0.1076                      & {\ul 0.0433}                                   & {\ul 0.0512}                &  0.0881& 0.1317& 0.0504& {\ul 0.0611}& {\ul 0.0291}                        & 0.0472                          & 0.0146             & 0.0171   \\
        MMSR (CIKM'23)                            & 0.0218          & 0.0322           & 0.0135          & 0.0142                     & 0.0715                      & 0.1062                      & 0.0401                      & 0.0446                      & 0.0878& 0.1367& 0.0505& 0.0601& 0.0245                            & 0.0456                          & 0.0129               & 0.0156  \\
        MMSBR (TKDE'23)                           & 0.0235          & 0.0325           & 0.0134          & {\ul 0.0158}               & 0.0727                      & 0.1088                      & 0.0427                      & 0.0504                      & 0.0865&  0.1325& 0.0503& 0.0599& 0.0271                            & 0.0464                          & {\ul 0.0151}         & 0.0181  \\
        MP4SR (TOIS'24)                           & 0.0223          & {\ul 0.0327}     & 0.0129          & 0.0155                     & 0.0731                      & {\ul 0.1092}              & 0.0425                      & 0.0511                      & 0.0898& 0.1321& 0.0509& 0.0604& 0.0281                            & {\ul 0.0483}                    & 0.0149               & {\ul 0.0186}  \\ \hline
        SG-UMP+SASRec                    & 0.0211          & 0.0299           & 0.0114          & 0.0141                     & 0.0688                      & 0.1043                      & 0.0356                      & 0.0443                      & 0.0960                       & 0.1423                     & 0.0527                    & 0.0640                       & 0.0267                            & 0.0435                          & 0.0137               & 0.0171  \\
        \emph{vs. Vanilla}              & 25.60\%         & 20.08\%          & 40.74\%         & 42.42\%                    & 28.84\%                     & 24.31\%                     & 44.13\%                     & 33.43\%                     & 12.54\%                      & 13.30\%                  & 8.21\%                 & 8.11\%                    & {14.59\%}                         & 11.25\%                         & 11.38\%              & 12.50\% \\
        SG-UMP+STOSA                     & 0.0242          & 0.0349           & 0.0144          & 0.0167                     & 0.0788                      & 0.1091                      & 0.0455                      & 0.0534                      & 0.0975                       & 0.1454                     & 0.0563                    & 0.0683                       & 0.0279                            & 0.0492                          & 0.0151               & 0.0184  \\
        \emph{vs. Vanilla}              & 43.20\%         & 32.20\%          & 46.94\%         & 47.79\%                    & 21.60\%                     & 15.94\%                     & 34.22\%                     & 38.70\%                     & 12.85\%                      & 13.24\%                  & 13.28\%                 & 13.46\%                    & 17.23\%                           & 16.04\%                         & 17.97\%              & 14.29\%     \\
        SG-UMP+Oracle4Rec                    & \textbf{0.0264} & \textbf{0.0361}  & \textbf{0.0165} & \textbf{0.0178}            & \textbf{0.0807}             & \textbf{0.1188}             & \textbf{0.0476}             & \textbf{0.0565}             & \textbf{0.1017}              & \textbf{0.1609}            & \textbf{0.0601}           & \textbf{0.0707}              & \textbf{0.0312}                   & \textbf{0.0516}                 & \textbf{0.0162}      & \textbf{0.0202}  \\
        \emph{vs. Vanilla}              & 25.12\%         & 20.86\%          & 25.95\%         & 23.61\%                    & 17.64\%                     & 19.16\%                     & 25.59\%                     & 25.28\%                     & 12.87\%                      & 13.39\%                  & 17.61\%                 & 15.90\%                    & 17.29\%                           & 15.96\%                         & 10.96\%              & 15.43\% \\ \hline
        \emph{vs. Best}                 & 11.39\%         & 10.40\%          & 13.79\%         & {12.66\%}                  & {9.80\%}                    & {8.79\%}                    & {9.93\%}                    & {10.35\%}                   & 12.87\%                     & 13.39\%                   & 17.61\%                  & 15.71\%                     & 7.22\%                            & 6.83\%                          & 7.28\%               & 8.60\% \\ \hline
        \end{tabular}
        }
    \vspace{-8pt}
\end{table*}
